On the Limiting Vacillating Tableaux for Integer Sequences

A fundamental identity in the representation theory of the partition algeba is $n^k = \sum_{\lambda} f^\lambda m_k^\lambda$ for $n \geq 2k$, where $\lambda$ ranges over integer partitions of $n$, $f^\lambda$ is the number of standard Young tableaux of shape $\lambda$, and $m_k^\lambda$ is the number of vacillating tableaux of shape $\lambda$ and length $2k$. Using a combination of RSK insertion and jeu de taquin, Halverson and Lewandowski constructed a bijection $DI_n^k$ that maps each integer sequence in $[n]^k$ to a pair consisting of a standard Young tableau and a vacillating tableau. In this paper, we show that for a given integer sequence $\boldsymbol{i}$, when $n$ is sufficiently large, the vacillating tableaux determined by $DI_n^k(\boldsymbol{i})$ become stable when $n \rightarrow \infty$; the limit is called the limiting vacillating tableau for $\boldsymbol{i}$. We give a characterization of the set of limiting vacillating tableaux and presents explicit formulas that enumerate those vacillating tableaux.

==> References.tex <==

% Keyword: Initiial + last two digit 

\begin{thebibliography}{99}

\bibitem{BH17} G. Benkart, T. Halverson. 
Partition Algebras and the Invariant Theory of the Symmetric Group. arXiv:1709.07751

\bibitem{BHH17} 
G. Benkart, T. Halverson, and N. Harman, Dimensions of irreducible modules for partition algebras and tensor power multiplicities for symmetric and alternating groups, 
\emph{J.
Algebr. Combin}. 46 no. 1 (2017), 77-108; arXiv:1605.06543.

\bibitem{CDDSY07} 
W.Y.C. Chen, E.Y.P. Deng, R.R.X.Du, R.P.Stanley and C.H. Yan.
{Crossings and nestings of matchings and set partitions }.  
\emph{Trans. Amer. Math. Soc}. volume 359, no. 4, (2007) 1555--1575.

\bibitem{COSSZ} LAURA COLMENAREJO, ROSA ORELLANA, FRANCO SALIOLA, ANNE SCHILLING, AND MIKE ZABROCKI,
AN INSERTION ALGORITHM ON MULTISET PARTITIONS WITH APPLICATIONS TO DIAGRAM ALGEBRAS, arXiv:1905.02071v2. 

\bibitem{GP11} 
A. M.Goyt and L.K. Pudwell. Solution to Monthly  problem 11567. May, 2011. 
 https://faculty.valpo.edu/lpudwell/papers/MonthlyStirling.pdf
 
\bibitem{HJ18} T. Halverson and T.N. Jacobson. 
Set-partition tableaux and representations of diagram algebras. arXiv:1808.08118. 




\bibitem{HL05} T.Halverson and  T. Lewandowski. 
RSK insertion for set partitions and diagram algebras.
\emph{Electron J. Combin.} 11 (2004/2006), 24. 

\bibitem{HT10} T. Halverson and N. Thiem. 
$q$-Partition algebra combinatorics. 
\emph{J. Cocmbin. Theory A}, 117(2010), 507--527. 

\bibitem{Kratten06} C. Krattenthaler. 
Growth diagrams, and increasing and decreasing chains in fillings of Ferrrers shapes. 
\emph{Adv. Appl. Math.} 37(2006), 404--431. 



\bibitem{OZ15} R. Orellana and M. Zabrocki, Symmetric group characters as symmetric functions,
arXiv:1605.06672v2. 

\bibitem{OEIS} N. J. A. Sloane. The On-line Encyclopedia of Integer Sequences. \url{https://oeis.org. } 

\bibitem{Sagan01} B. Sagan. the Symmetric Groups, Representations, Combinatorial Algorithms, and Symmetric Functions, second edition, Springer-Verlag, New York, 2001. 


\bibitem{EC2} R. Stanley. Enumerative Combinatorics, Vol. 2, Cambridge University Press, Cambridge, 1999. 

\bibitem{Sunderam90} 
S. Sundaram, The Cauchy identity for Sp(2n), J. Combin. Theory Ser. A, 53 (1990), 209–238.
\end{thebibliography}


